Electron-positron pair production in inhomogeneous electromagnetic fields

The process of electron-positron pair production is investigated within the phase-space Wigner formalism. The similarities between atomic ionization and pair production for homogeneous, but time-dependent linearly polarized electric fields are examined mainly in the regime of multiphoton absorption (field-dependent threshold, above-threshold pair production). Characteristic signatures in the particle spectra are identified (effective mass, channel closing). The non-monotonic dependence of the particle yield on the carrier frequency is discussed as well. The investigations are then extended to spatially inhomogeneous electric fields. New effects arising due to the spatial dependence of the effective mass are discussed in terms of a semi-classical interpretation. An increase in the normalized particle yield is found for various field configurations. Pair production in inhomogeneous electric and magnetic fields is also studied. The influence of a time-dependent spatially inhomogeneous magnetic field on the momentum spectrum and the particle yield is investigated. The Lorentz invariants are identified to be crucial in order to understand pair production by strong electric fields in the presence of strong magnetic fields.

==> pre_chap6.tex <==
\pagestyle{fancy}

In Fig. \ref{Fig_YieldFull} we have illustrated the particle yield as a function of the field frequency. To do this, we employed a generic, pulsed electric field superimposed by a photon-energy dependent subcycle structure.

In total, we differentiate between three different regimes. In case of low field frequencies $\omega$ Schwinger pair production dominates. The increase in the particle yield is due to the fact, that in the tunneling regime the pulse length is a major factor when determining the production rate. The lower $\omega$ the fewer oscillations in the field, thus the time interval the field is close to its peak value is extended. We also observe, that in Fig. \ref{Fig_YieldFull} the yield is noisy in the midrange. As the pulse length is finite, there is a regime where the employed electric field is basically a few-cycle pulse. Interpretation of the momentum output in the case of a few-cycle pulse is complicated and beyond the scope of this thesis. However, we will give example results in section \ref{App_CEP}. Of major importance in the chapters five and six is the high-frequency sector, thus the regime of multiphoton pair production. In this region the electric field is a many-cycle pulse exhibiting an oscillatory structure mimicking a monochromatic pulse.

\begin{figure}[hb]
\begin{center}
  \includegraphics[width=0.9\textwidth]{./Fig/QKT/pic3_0_1b}
\end{center}
  \renewcommand\thefigure{I}
\caption[Particle yield as a function of the field frequency.]{Logarithmic plot of the particle yield $N$ for various field frequencies $\omega$ for a pulse with finite temporal extent. The drop off at $\omega \sim 0.1$ $m$ signals a transition from a Schwinger dominated region($\omega \lesssim 0.1$ $m$) to an absorption dominated region($\omega \gtrsim 0.1$ $m$). The clear peaks in the region $\omega \ge 0.5$ $m$ are characteristically for multiphoton pair production in many-cycle pulses. Parameters: Tab. \ref{Tab_EffM1_App}} 
\label{Fig_YieldFull}
\end{figure}
